Pick and Place Planning is Better than Pick Planning then Place Planning

Robotic pick and place stands at the heart of autonomous manipulation. When conducted in cluttered or complex environments robots must jointly reason about the selected grasp and desired placement locations to ensure success. While several works have examined this joint pick-and-place problem, none have fully leveraged recent learning-based approaches for multi-fingered grasp planning. We present a modular algorithm for joint pick and place planning that can make use of state of the art grasp classifiers for planning multi-fingered grasps for novel objects from partial view point clouds. We demonstrate our joint pick and place formulation with several costs associated with different placement tasks. Experiments on pick and place tasks with cluttered scenes using a physical robot show that our joint inference method is more successful than a sequential pick then place approach, while also achieving better placement configurations.

==> Implementation.tex <==
\section{Implementation}

==> intro-fig.tex <==
\setcounter{figure}{1}
\makeatletter
\let\@oldmaketitle\@maketitle% Store \@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle% Update \@maketitle to insert...
  \begin{center}
      %\includegraphics[width=\textwidth/\real{3}, trim={500, 185, 85, 160}, clip]{/Figures/IntroSketch/mast_place_2.jpg}\hspace{-3.75pt}
      %\includegraphics[width=\textwidth/\real{3}, trim={500, 185, 85, 160}, clip]{/Figures/IntroSketch/mast_place_3.jpg}\hspace{-3.75pt}
      %\includegraphics[width=\textwidth/\real{3}, trim={500, 185, 85, 160}, clip]{/Figures/IntroSketch/mast_place_1.jpg}
      %\includegraphics[width=0.5\textwidth, trim={480, 155, 75, 230}, clip]{/Figures/IntroSketch/mast_grasp_2.jpg}\hspace{-4pt}
      %\includegraphics[width=0.5\textwidth, trim={480, 155, 75, 230}, clip]{/Figures/IntroSketch/mast_grasp_1.jpg}
      \includegraphics[width=\textwidth, trim={90, 115, 90, 115}, clip]{/Figures/IntroSketch/IntroFigure.pdf}
  \end{center}
  %\refstepcounter{figure}
  \vspace{-10pt}
  \footnotesize{\textbf{Fig.~\thefigure:\label{fig:mast}}~Examples illustrating effects of grasp and placement configurations for placing into clutter. \textbf{Left \& Middle:} Multiple grasp and place configurations for the same pick and place task.  \textbf{Left:} Different successful grasp solutions for the same object (top grasp: green, side grasp: red). \textbf{Middle:} Corresponding place configurations: place for side grasp configuration (red) is infeasible due to the robot in collision, place configuration for top grasp (green) is feasible. \textbf{Right:} Reachability effects of grasp choice:  \textbf{Right-Top:} Unable to reach target behind red can due to limited reachability with top grasp. \textbf{Right-Bottom} Target reached with side grasp. }% CAPTION
 \vspace{-24pt}
  \medskip}% ... an image
\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> pick_n_place_alg.tex <==
\begin{algorithm}\label{alg:pick-n-place}
  \caption{Pick and Place for Object Sequences}
  \begin{algorithmic}[1]
    \Procedure{Pick\_N\_Place}{$Z_E,\mathcal{Z}_O = [Z_O^{1},\ldots]$}
    \State \( \mathcal{D} \leftarrow \left[\builddsdf(Z_E)\right]\) \label{alg:dsdf-init}
    \For{each $Z_O$ in \(\mathcal{Z}_O\)} // Plan for each object
    \State \( q \leftarrow \texttt{PriorityQueue()}\)
    \For{$i$ in \(\texttt{MDN}(Z_O).num\_components\)}
    \State \(\thetav_{g}^0 \leftarrow \sim \texttt{MDN}(Z_O, i)\) \label{alg:sample-grasp}
    \State \(\xv_{p}^0 \leftarrow \sim \nabla \mathcal{D} == 0\) \label{alg:sample-init-place}
    \State $\xv_p, \thetav_g, c \leftarrow \texttt{Optimize}(Z_O, \mathcal{D}, \thetav_{g}^0, \xv_{p}^0)$\label{alg:opt-line}
    \State $q.\texttt{push}((\xv_{p}, \thetav_{g}), c)$\label{alg:push-q}
    \EndFor\label{alg:end-plan}
    \While{$!\placed$} // Execute pick and place \label{alg:exec-loop}
    \If{\(q.\)\texttt{empty}()}
    \State \Break
    \EndIf
    \State \(\xv_{p}^*, \thetav_{g}^* \leftarrow q.\texttt{pop}()\)\label{alg:pop-q}
    \If{$!\texttt{has\_plan}(Z_O, \mathcal{D}, \thetav_{g}^*, \xv_{p}^*)$}\label{alg:plan-trajectory}
    \State \Continue
    \EndIf
    \If{$!\texttt{execute\_grasp}(\thetav_{g}^*, Z_O)$}\label{alg:execute-grasp}
    \State \Continue
    \EndIf
    \If{!$\texttt{execute\_place}()$}\label{alg:execute-place}
    \State \Break
    \EndIf
    \State \(\mathcal{D}\texttt{.append}(\builddsdf(Z_0(\xv_p^*))\)\label{alg:add-dsdf} % Add DSDF of E build on input, append to list here
    \State \(\placed \leftarrow \texttt{true}\)
    \EndWhile \label{alg:end-exec-while}
    \EndFor
    \EndProcedure
  \end{algorithmic}
  \label{alg:pick-n-place}
\end{algorithm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

